The Poincar\'e pear and Poincar\'e-Darwin fission theory in astrophysics, 1885-1901

In the early 1880s, Henri Poincar\'e discovered a new equilibrium figure for uniformly-rotating fluid masses -- the pear, or piriform figure -- and speculated that in certain circumstances the pear splits into two unequal parts, and provides thereby a model for the origin of binary stars. The contemporary emergence of photometric and spectroscopic studies of variable stars fueled the first models of eclipsing binaries, and provided empirical support for a realist view of equilibrium figures -- including the pear -- in the cosmic realm. The paper reviews astrophysical interpretation of the Poincar\'e pear and the Poincar\'e-Darwin fission hypothesis with respect to research on variable stars from 1885 to 1901.

==> babelbst.tex <==
%%% babelbst.tex, modified by saw: addition of \bbled \bbleds \bbledby
%%% Bibliographieuebersetzungen:
%%%   english
%%%   german
%%%   ngerman
%%%
\newcommand *\englishbibnames {%
  \newcommand *\bbland        {and}%
  \newcommand *\bblapr        {april}%
  \newcommand *\bblaug        {august}%
  \newcommand *\bblchapter    {chapter}%
  \newcommand *\bbldec        {december}%
  \newcommand *\bbledition    {edition}%
  \newcommand *\bbleditor     {editor}%
  \newcommand *\bbleditors    {editors}%
  \newcommand *\bbleds        {eds}%
  \newcommand *\bbled         {ed}%
  \newcommand *\bbledby       {edited by}%
  \newcommand *\bblet         {et}%
  \newcommand *\bbletal       {\bblet\ al.}%
  \newcommand *\bblfeb        {february}%
  \newcommand *\bblin         {in}%
  \newcommand *\bbljan        {january}%
  \newcommand *\bbljul        {july}%
  \newcommand *\bbljun        {june}%
  \newcommand *\bblmar        {march}%
  \newcommand *\bblmay        {may}%
  \newcommand *\bblmthesis    {master's thesis}%
  \newcommand *\bblnov        {november}%
  \newcommand *\bblno         {\textnumero }%
  \newcommand *\bblnumber     {number}%
  \newcommand *\bbloct        {october}%
  \newcommand *\bblof         {of}%
  \newcommand *\bblpage       {page}%
  \newcommand *\bblpages      {pages}%
  \newcommand *\bblphdthesis  {Ph.D.~dissertation}%
  \newcommand *\bblsep        {september}%
  \newcommand *\bbltechreport {Technical report}%
  \newcommand *\bblvolume     {Volume}%
  }%
\newcommand *\frenchbibnames {%
  \newcommand *\bbland        {et}%
  \newcommand *\bblapr        {avril}%
  \newcommand *\bblaug        {ao\^ut}%
  \newcommand *\bblchapter    {chapitre}%
  \newcommand *\bbldec        {d\'ecembre}%
  \newcommand *\bbledition    {\'edition}%
  \newcommand *\bbleditor     {dir}%
  \let \bbleditors = \bbleditor
  \let \bbleds = \bbleditor
  \let \bbled = \bbleditor
  \newcommand *\bbledby       {publi\'e par}%
  \newcommand *\bblet         {\textit{\&}}%
  \newcommand *\bbletal       {et.\,al.}%
  \newcommand *\bblfeb        {f\'evrier}%
  \newcommand *\bblin         {in}%
  \newcommand *\bbljan        {janvier}%
  \newcommand *\bbljul        {juillet}%
  \newcommand *\bbljun        {juin}%
  \newcommand *\bblmar        {mars}%
  \newcommand *\bblmay        {mai}%
  \newcommand *\bblmthesis    {Th\`ese de master}%
  \newcommand *\bblphdthesis  {Th\`ese de doctorat}%
  \newcommand *\bblnov        {novembre}%
  \newcommand *\bblno         {N\mbox{$^\circ$}}%
  \newcommand *\bblnumber     {nombre}%
  \newcommand *\bbloct        {octobre}%
  \newcommand *\bblof         {de}%
  \newcommand *\bblpage       {page}%
  \newcommand *\bblpages      {pages}%
  \newcommand *\bblp          {p.}%
  \newcommand *\bblpp         {p.}%
  \newcommand *\bblsep        {septembre}%
  \newcommand *\bbltechreport {rapport technique}%
  \newcommand *\bblvolume     {T.}%
  }%
\newcommand *\germanbibnames {%
  \newcommand *\bbland        {und}%
  \newcommand *\bblapr        {April}%
  \newcommand *\bblaug        {August}%
  \newcommand *\bblchapter    {Kapitel}%
  \newcommand *\bbldec        {Dezember}%
  \newcommand *\bbledition    {Auflage}%
  \newcommand *\bbleditor     {Herausgeber}%
  \let \bbleditors = \bbleditor
  \let \bbleds = \bbleditor
  \let \bbled = \bbleditor
  \newcommand *\bbledby       {Hrsg. von}%
  \newcommand *\bblet         {\textit{\&}}%
  \newcommand *\bbletal       {u.\,a.}%
  \newcommand *\bblfeb        {Februar}%
  \newcommand *\bblin         {in}%
  \newcommand *\bbljan        {Januar}%
  \newcommand *\bbljul        {Juli}%
  \newcommand *\bbljun        {Juni}%
  \newcommand *\bblmar        {M\"arz}%
  \newcommand *\bblmay        {Mai}%
  \newcommand *\bblmthesis    {\glqq Master\grqq-Abschlu\ss{}arbeit}%
  \newcommand *\bblphdthesis  {Doktorarbeit}%
  \newcommand *\bblnov        {November}%
  \newcommand *\bblno         {Nr.}%
  \newcommand *\bblnumber     {Nummer}%
  \newcommand *\bbloct        {Oktober}%
  \newcommand *\bblof         {von}%
  \newcommand *\bblpage       {Seite}%
  \newcommand *\bblpages      {Seiten}%
  \newcommand *\bblsep        {September}%
  \newcommand *\bbltechreport {Technischer Bericht}%
  \newcommand *\bblvolume     {Band}%
  }%
\let \ngermanbibfixes = \relax
\iflanguage {english}{%
  \englishbibnames
  }{\iflanguage {french}{%
    \frenchbibnames
    }{\iflanguage {german}{%
      \germanbibnames
      }{\iflanguage {ngerman}{%
        \germanbibnames
        \ngermanbibfixes
        }{%
        \message {^^JSprache undefiniert in babelbst.tex f\"ur Befehl \string#1.^^J}}}}}%

